Can Quantum Communication Speed Up Distributed Computation?

The focus of this paper is on {\em quantum distributed} computation, where we investigate whether quantum communication can help in {\em speeding up} distributed network algorithms. Our main result is that for certain fundamental network problems such as minimum spanning tree, minimum cut, and shortest paths, quantum communication {\em does not} help in substantially speeding up distributed algorithms for these problems compared to the classical setting. In order to obtain this result, we extend the technique of Das Sarma et al. [SICOMP 2012] to obtain a uniform approach to prove non-trivial lower bounds for quantum distributed algorithms for several graph optimization (both exact and approximate versions) as well as verification problems, some of which are new even in the classical setting, e.g. tight randomized lower bounds for Hamiltonian cycle and spanning tree verification, answering an open problem of Das Sarma et al., and a lower bound in terms of the weight aspect ratio, matching the upper bounds of Elkin [STOC 2004]. Our approach introduces the {\em Server model} and {\em Quantum Simulation Theorem} which together provide a connection between distributed algorithms and communication complexity. The Server model is the standard two-party communication complexity model augmented with additional power; yet, most of the hardness in the two-party model is carried over to this new model. The Quantum Simulation Theorem carries this hardness further to quantum distributed computing. Our techniques, except the proof of the hardness in the Server model, require very little knowledge in quantum computing, and this can help overcoming a usual impediment in proving bounds on quantum distributed algorithms.

==> techniques_overview.tex <==
\vspace{-0.1in}
\section{Overview of Technical Approach}\label{sec:technique}

\begin{figure*}
\center
%\tiny
%\includegraphics[width=\linewidth, clip=true, trim= 0cm 3cm 0cm 3cm]{proof_structure.pdf}\\
%
\begin{tikzpicture}[auto, node distance=0.1cm]
\scriptsize
\node (xor) [rectangle, draw=black, text centered, text=black, text width=2cm] {XOR games};
\node (and) [rectangle, draw=black, text centered, text=black, text width=2cm, below=1 of xor] {AND games};
\node (ipthree_server) [rectangle, draw=black, text centered, text=black, right=1 of xor, text width=3cm] {$\ipmodthree_n$ \\ {two-sided error, server model}};
\node (disj_server) [rectangle, draw=black, text centered, text=black, right=1 of and, text width=3cm] {$(\beta n)-\eq_n$\\ {one-sided error, server model}};
%
\node (ham_server) [rectangle, draw=black, text centered, text=black, right=1 of ipthree_server, text width=3cm] {$\ham_n$ \\ {two-sided error, server model}};
\node (conn_server) [rectangle, draw=black, text centered, text=black, right=1 of disj_server, text width=3cm] {$(\beta n)-\ham_n$ \\ {one-sided error, server model}};
%
\node (ham_distributed) [rectangle, draw=black, text centered, text=black, right=1.4 of ham_server, text width=3cm] {$\ham$ \\ {two-sided error, distributed network}};
\node (conn_distributed) [rectangle, draw=black, text centered, text=black, right=1.4 of conn_server, text width=3cm] {$\alpha$-approx $\mst$ \\ {Monte Carlo, distributed network}};
%
\node (ham_cc) [rectangle, draw=gray, text centered, text=gray, above=0.3 of ham_server, text width=3cm] {$\ham_n$ \\ {two-sided error, communication complexity}};
\node (conn_cc) [rectangle, draw=gray, text centered, text=gray, below=0.3 of conn_server, text width=3cm] {$(\beta n)-\ham_n$ \\ {one-sided error, communication complexity}};
%
\node (disj_cc) [rectangle, draw=gray, text centered, text=gray, below=0.3 of disj_server, text width=3cm] {$(\beta n)-\eq_n$\\ {one-sided error, communication complexity}};
%
\draw[->, thick, black] (xor.east) -- node [midway] {Sec~\ref{sec:basic lower bounds server model}}  (ipthree_server.west);
\draw[->, thick, black] (ipthree_server.east) -- node [midway] {Sec~\ref{sec:server graph}}  (ham_server.west);
\draw[->, thick, black] (ham_server.east) -- node [midway] {Sec~\ref{sec:from server to distributed},\ref{sec:proof of main}} (ham_distributed.west);
%
%\draw[->, thick, black] (xor.east) -- ++(0.5, 0) |- node [midway] {Sec~\ref{sec:basic lower bounds server model}} (disj_server.west);
\draw[->, thick, black] (and.east) -- node [midway] {Sec~\ref{sec:basic lower bounds server model}}  (disj_server.west);
\draw[->, thick, black] (disj_server.east) -- node [midway] {Sec~\ref{sec:server graph}} (conn_server.west);
\draw[->, thick, black] (conn_server.east) --  node [midway] {Sec~\ref{sec:from server to distributed},\ref{sec:proof of main}} (conn_distributed.west);
%
\draw[->, gray] (ham_server.north) -- (ham_cc.south);
\draw[->, gray] (conn_server.south) -- (conn_cc.north);
%
\draw[->, gray] (disj_server.south) -- (disj_cc.north);
%
  \node (nonlocal) [above=1 of xor, text width=2cm, text centered, text=blue] {{\bf Nonlocal Games}};
  \draw [-, dashed, blue] ([xshift=0.6cm] nonlocal.east) -- ++(0, -5);
  \node (server) [right=3 of nonlocal, text width=2cm, text centered, text=blue] {{\bf Server Model}};
  \draw [-, dashed, blue] ([xshift=4cm] server.east) -- ++(0, -5);
  \node (distributed) [right=5 of server, text width=2cm, text centered, text=blue] {{\bf Distributed Networks}};
\end{tikzpicture}
\caption{Our proof structure. Lines in gray show the implications of our results in communication complexity.}\label{fig:proof structure}
\end{figure*}

The high-level idea behind our lower bound proofs is by establishing a connection between
quantum communication complexity and quantum distributed network computing.
Our work is inspired by \cite{DasSarmaHKKNPPW11} (following a line of work in \cite{PelegR00,LotkerPP06,Elkin06,KorKP11}) which shows lower bounds of many graph verification and optimization problems in the {\em classical} distributed computing model.
%, including tight randomized  lower bounds for connectivity verification.
%
%and approximating the minimum spanning tree and deterministic tight lower bounds of Hamiltonian cycle and spanning tree verification.
%
The main technique used to show the classical lower bounds in \cite{DasSarmaHKKNPPW11} is
 the {\em Simulation Theorem} (cf. Theorem 3.1 in \cite{DasSarmaHKKNPPW11}) which shows how one can use
lower bounds for problems in the standard two-party (Yao's) classical communication complexity model \cite{KNbook} to derive lower bounds of equivalent problems in the ``distributed'' version of communication complexity. Specifically, the Simulation Theorem   relates the {\em communication} lower bound from the standard two-party  communication complexity model to compute some appropriately chosen function $f$ (e.g., Set Disjointness or Equality) to the distributed {\em time} complexity lower bound for computing the same function in a specially chosen graph $G$. They use a graph  that was first used in  \cite{PelegR00}. The Simulation Theorem effectively  reduces the task of proving lower bounds of {\em graph verification} problems to merely picking the right function $f$ to reduce from. Two functions
that were used in \cite{DasSarmaHKKNPPW11} were Set Disjointness and Equality, which are  quintessential problems in the world of communication complexity \cite{KNbook}.
Finally, one can reduce the verification problem to hardness of distributed approximation for a variety of problems to show that the same lower bounds hold for approximation algorithms as well.
% which shows that the complexity behind a complicated network structure is captured by the standard two-party communication complexity; thus showing distributed algorithm lower bounds is no harder than showing a communication complexity.
%
% of set disjointness ($\disj_n$).
%
Our starting point for showing lower bounds for the quantum setting is a question whether there is a {\em quantum} version of the Simulation Theorem, i.e., whether one can prove quantum distributed algorithm lower bounds via quantum (two-party) communication complexity lower bounds.   However, this seems challenging to do due to  several difficulties  (as explained below); in fact, it leads us to a proof
that is substantially different compared to the classical setting. In particular, while we cannot prove a ``quantum" Simulation Theorem using the standard two-party model, we manage to identify a new communication model called the {\em server} communication model and  prove a server model version of the Simulation Theorem. Our new Simulation Theorem shows that the server model captures the hardness of distributed algorithms well in both the classical and quantum setting. We then show that many important bounds in the standard quantum two-party model also hold in the server model. Some of the bounds we prove are even new in the standard model and classical setting. These bounds together with our new Simulation Theorem lead to our main results. Details are as follows.


%In particular, our reduction uses a newly introduced communication complexity model called the {\em server} model, and we prove several new bounds in this model which also imply some new lower bounds in the two-party model. Details are as follows.

%introducing a new model called the {\em server} model which is closely related to the two-party model

%\paragraph{Two-Party Communication Complexity, Simulation Theorem and Server Model}
\paragraph{Where the Simulation Theorem Fails and the Server Model Helps}
The first difficulty in extending previous techniques is that is it not clear whether the Simulation Theorem holds in the quantum setting (i.e., whether a quantum two-party communication complexity implies a distributed algorithm lower bound). The main reason is that its proof seems to require the two players, say Alice and Bob, to simulate some common nodes in a network. While this is easy to do in the classical setting, it is not clear whether it is still possible in the quantum setting.

To illustrate this point, let us introduce a new model called the {\em server} model. There are three players in the server model, Carol, David and the server. Carol and David receive the inputs $x$ and $y$, respectively, and want to compute $f(x, y)$ for some function $f$. As in the two-party model, Carol and David can talk to each other. Additionally, they can talk to the server. The catch here is that the server can send messages for {\em free}. Thus, the communication complexity in the server model counts only messages sent by Carol and David. This model, even without prior entanglement, is clearly at least as strong as the standard quantum communication complexity model with shared entanglement, since the server can dispense any entangled state to Carol and David.

%However, they cannot communicate directly to each other but they have to send a message to the server. The server, after receiving a message from both sides, will send a message back to the players. This protocol repeats until all parties stop with an answer. Our goal is to minimize the number of messages sent by the players to the server. The message sent by the server is {\em free}.

%Putting this model into a perspective,
%Looking back with the server model at hand, previous proof of the Simulation Theorem can be viewed as composing of two separate ideas. The first idea is to show a lower bound

With the server model in our perspective, we can refine the previous connection between two-party communication complexity and distributed algorithm lower bound (i.e., the Simulation Theorem) to two separate connections: (1) A connection between the two-party and server models and (2) A connection between the server model and distributed networks. We will show that the second connection holds even in the quantum setting with entanglement: %(see Section~\ref{sec:from server to distributed})

\begin{theorem}[Details in Section~\ref{sec:from server to distributed}]%\label{theorem:from server to distributed}
For any $B$, $L$, $\Gamma\geq \log L$, $\beta\geq 0$ and $\epsilon_0, \epsilon_1>0$, there exists a $B$-model quantum network $N$ of diameter $\Theta(\log L)$ and $\Theta(\Gamma L)$ nodes such that if $Q_{\epsilon_0, \epsilon_1}^{*, N}((\beta\Gamma)\mbox{-}\ham(N))\leq \frac{L}{2}-2$ then $Q_{\epsilon_0, \epsilon_1}^{*, \server}((\beta\Gamma)\mbox{-}\ham_\Gamma)= O((B\log L)Q_{\epsilon_0, \epsilon_1}^{*,N}((\beta\Gamma)\mbox{-}\ham(N)))$. \end{theorem}

This theorem is similar to the Simulation Theorem in \cite{DasSarmaHKKNPPW11} except that it replaces the standard two-party model by the server model.
\iffalse
Our proof follows from previous techniques  \cite{PelegR00,LotkerPP06,Elkin06,KorKP11,DasSarmaHKKNPPW11,NanongkaiDP11} (e.g., we use a similar graph and maintain the state of similar sets of nodes) but also provides some simplification (e.g., we reduce from graph problems directly, leaving most of the ``hard part" in the communication complexity model, and we do not require simulating common nodes which is a source of confusion). This proof also shows that the underlying idea of this technique is in fact the same as the simple idea of {\em bisection width} commonly used in distributed networking as well as other areas (see, e.g., \cite{KNbook,Leighton91,KuhnO11,FrischknechtHW12}).
Now we know that the second connection holds even in the quantum setting.
\fi
 To prove the quantum version of the Simulation Theorem, it remains to show the first connection: the server-model communication complexity is lower bounded by the two-party communication complexity.
%
%This is where one of the main difficulties lie in: {\em While it is easy to prove that the two models are equivalent in the classical setting, it is not clear if they are in the quantum setting.} Let us now explain this.
%
%Clearly, the communication complexity of the server model is {\em at most} the two-party model, even in the quantum setting with prior entanglement since Carol and David can pretend to be Alice and Bob.
%%
%%, since Carol, David and the server can simulate a two-party protocol by pretending to be Alice, Bob and a communication channel respectively (i.e., the server will simply forward the messages between Carol and David).
%%
%%(1) complexity(Server model)\leq complexity(two-party models)
%%
%Is the communication complexity of the server model substantially smaller than the two-party model? We believes that this is not the case. Since the server does not get any input, he seems to act only as a channel; so, it is quite intuitive that the communication complexity in the server model should be asymptotically the same as in the two-party model.
%
We note that it is clear that the converse is true: the communication complexity of the server model is {\em at most} the two-party model in both classical and quantum settings since Carol and David can pretend to be Alice and Bob. On the other hand, it is conceivable the two models are equivalent: Since the server does not get any input, he seems to act only as a channel.  While it is easy to prove that the two models are equivalent in the classical setting (see proof sketch in Appendix), it is not clear if they are in the quantum setting.
%
%While it is easy to show that the two models are equivalent in the classical setting, it seems quite nontrivial to prove or disprove this in the quantum setting.

%is actually the case in the classical setting. Its proof is so simple that we can sketch it now.
\iffalse
To explain some issues in the quantum setting, let us sketch the proof of this in the classical setting. Let us first consider the deterministic setting. The proof is by the following ``simulation'' argument. Alice will simulate Carol and the server. Bob will simulate David and the server. In each round, Alice will see all messages sent from the server to Carol and thus she can keep simulating Carol. However, she does not see the message sent from David to the server which she needs to simulate the server. So, she must get this message from Bob. Similarly, Bob will get from Alice the message sent from Carol to the server. These are the only messages we need in each round in order to be able to simulate the protocol. Observe that the total number of bits sent between Alice and Bob is exactly the number of bits sent by Carol and David to the server. Thus, the complexities of both models are exactly the same in the deterministic case.
We can conclude the same thing for the public coin setting (where all parties share a random string) since Alice and Bob can use their shared coin to simulate the shared coin of Carol, David and the server.

{\bf Gopal:}- In the above, technically, should we not count the bits sent by Carol and David directly to each other also?

The above argument, however, does not seem to work in the quantum setting. The main issue with a simulation along the lines of the one sketched above is that Alice and Bob cannot simulate a ``copy'' of the server each.
For instance one could try to simulate the server's state in a distributed way by maintaining the state that results by applying CNOT to every qubit of the server and a fresh qubit, and distribute these qubits to Alice and Bob. But then if the server sends a message to Carol, Bob would have to disentangle the corresponding qubits in his copy, which would require a message to Alice.

 %is that it is impossible for Alice and Bob to simulate the server at the same time without communication. For example, if they want to simulate a measurement operation of the server, they cannot simply do a measurement separately since they could get a different result. Thus, it is conceivable that if the server makes server measurements then Alice and Bob have to communicate a lot to ``synchronize'' their measurement results.


%Another evidence that makes it possible that the two models are different in the quantum setting is that some techniques used to prove quantum lower bounds in the two-party model do not extend to the server model.\danupon{Is this really correct?} %For example, Kremer-Yao's decomposition \cite{Yao93,Kremer95} which are an important part of many proofs does not work in the server model.
\fi

While we leave this as an open question, we prove that many lower bounds in the two-party model extend to the server model.

%One of the troubles is this: In the argument above, Alice has to tell Bob the message that Alan sends to Referee so that Bob can simulate Referee. However, she also needs this message herself since she also needs to simulate Referee. If this message consists of qubits then this might be possible since Alice will lose what she sent to Bob (since she cannot clone the message).


%It generalizes the standard model with entanglement (Referee can dispense an arbitrary amount of entanglement). Intuitively it shouldn't be more powerful. I thought a bit about a simulation, maybe by compressing Referee's messages in the presence of entanglement, but didn't get anywhere.




\paragraph{Server-model Communication Complexity} (Details in Section~\ref{sec:basic lower bounds server model} and \ref{sec:server graph}) In this paper we show lower bounds of two types of problems. The first type consists of basic problems studied in the standard two-party model such as Equality and Set Disjointness. To show lower bounds of these problems, we show a connection between the server model and {\em nonlocal games}.
%
%, defined as follows.
%
%The first type of problems are those related to {\em block composed} functions.
%
Nonlocal games are games where Alice and Bob receive an input $x$ and $y$ from some distribution and want to compute $f(x, y)$. However, they cannot talk to each other. Instead, they output one bit, say $a$ and $b$, which are then combined to be an output. For example, in {\em XOR games} and {\em AND games}, these bits are combined as $a\oplus b$ and $a\wedge b$, respectively. The players' goal is to maximize the probability that the output is $f(x, y)$.
%
We relate nonlocal games to the server model by showing that the XOR- and AND-game players can use an efficient server-model protocol to guarantee a good winning chance.


%\danupon{This is from other section. Should rephrase or remove it from the other section} The local game is played by two players, say Alice and Bob. It consists of input domain $\iset=\{(x, y)\}$ and boolean functions $f: \iset\rightarrow \{0, 1\}$ and $g: \{0, 1\}^2\rightarrow \{0, 1\}$. We begin the game by drawing an input $(x, y)$ from a distribution $\pi$ (known to the Alice and Bob). After receiving an input each player must output a single bit, say $a$ and $b$. The output of the game is $g(a, b)$. For example, the output of the game will be $a\wedge b$ if $g$ is the AND function and $a\oplus b$ if $g$ is the XOR function. The players win the game if the output $g(a, b)$ is the same as $f(x, y)$. The goal of the players is to maximize the winning probability. Two games of our interest are {\em XOR}- and {\em AND}-games where $g$ is XOR and {\em AND} functions, respectively.
%%
%We relate nonlocal games to the server model by showing that that the XOR- and AND-game players can make use of an efficient server-model protocol to guarantee a good winning probability.

\begin{lemma}[Details in Section~\ref{sec:basic lower bounds server model}] For any boolean function $f$ and $\epsilon_0, \epsilon_1\geq 0$, there is an XOR-game strategy $\cA'$ and AND-game strategy $\cA''$ such that, for any input $(x, y)$, with probability $4^{-2Q^{*, \server}_{\epsilon_0, \epsilon_1}(f)}$, $\cA'$ and $\cA''$ output $f(x, y)$ with probability at least $1-\epsilon_{f(x,y)}$; otherwise $\cA'$ outputs $0$ and $1$ with probability $1/2$ each, and $\cA''$ outputs $0$ with probability $1$.
\end{lemma}
%
Following the $\gamma_2$-norm techniques in \cite{LinialS09,Sherstov11,LeeZ10} and the recent method of \cite{fooling12}, we show one- and two-sided error lower bounds of many problems on the server model, which match the two-party model lower bounds.

The second type of problems are graph problems. To show a lower bound of Hamiltonian cycle verification ($\ham_n$), we derive  reductions (using some novel gadgets) from {\em Inner Product mod 3} ($\ipmodthree_n$) and {\em Gap Equality} (\gap-$\eq_n$), defined in Section~\ref{sec:basic lower bounds server model}.  This result also implies a lower bound for spanning tree ($\st_n$) verification. (We note again that the lower bounds of $\ham_n$ and $\st_n$ are new even in the classical two-party model.)
%
%To show a lower bound of a gap version of connectivity verification ($\gap-\conn_n$), we show that previous reduction \cite{DasSarmaHKKNPPW11}\danupon{Also \cite{BabaiFS86}} preserves the gap.
%
Using the server-model communication complexity of $\ham_n$ and $\gap$-$\ham_n$, we can show lower bounds of distributed algorithms as discussed earlier. Fig.~\ref{fig:proof structure} depicts our proof strategy.





%
%\subsection{Related work}
%
%%\subsubsection{Quantum Communication Complexity}
%
%\paragraph{Quantum Communication Complexity of Disjointness.}\danupon{This is from Hartmut's earlier note. Note that the notation is slightly different: I use $Q_{\epsilon_0, \epsilon_1}$ while Hartmut uses $Q_{\epsilon_1, \epsilon_0}$.} Previous results about the disjointness problem are: \cite{BabaiFS86} prove $R^{cc}_\epsilon(\disj_n) = \Omega(\sqrt{n})$\danupon{Should we specify $\epsilon$?} and observe that $\disj_n$ is complete for the communication complexity version of co-NP. \cite{KalyanasundaramS92} and later \cite{Razborov92} prove the tight $\Omega(n)$ bound.  \cite{Razborov03} shows the tight $\Omega(\sqrt{n})$ lower bound for quantum protocols. This result was reproved in a simpler way in \cite{Sherstov11}. \cite{AaronsonA05} give a $O(\sqrt{n})$ upper bound for quantum protocols.  The bound from \cite{Razborov03} also holds in the model with prior entanglement. Hoyer and de Wolf \cite{HoyerW02} show that $Q^{cc}_{0, 1/2}(\disj_n) = n+1$ (no prior entanglement is allowed for this result).
%%
%Also note that the protocol in \cite{AaronsonA05} shows that $Q^{cc}_{1/3, 0} (\disj_n) = O(\sqrt{n})$.
%
%
%Thus, prior to this paper, we know that for some $\epsilon$,\danupon{Should we specify $\epsilon$?} $Q^{cc}_{\epsilon,0}(\disj_n)=Q^{*,cc}_{\epsilon,0}(\disj_n)=Q^{cc}_\epsilon(\disj_n)=Q^{*, cc}_\epsilon(\disj_n) = \Theta(\sqrt{n})$, $Q^{cc}_{0, \epsilon} (\disj_n) = \Theta(n)$, leaving the case of $Q^{*, cc}_{0, \epsilon} (\disj_n)$ as the only unknown case. One additional result of this paper closes this gap.
%
%
%For $\gap-\disj_n$, the fact that $R_{0, 1/2}((\beta n)-\disj_n)=\Theta(n)$ for some $\beta>1$ follows from the fact that $R_{0, 1/2}((\beta n)-\eq_n)=\Theta(n)$ \cite{BlaisBM11}. We are not aware of any result in the quantum setting prior to this paper. The result in this paper implies that $Q^{*, cc}_{0, 1/2}((\beta n)-\disj_n)=\Theta(n)$.

%\iffalse


%\paragraph{From Nayak-Salzman STOC'02} Note that there is no loss  of generality  in not allowing
%the players to measure a subset of their quantum bits in
%the intermediate  steps of  a  protocol.   This  is  because  all
%measurements may be postponed to the end by the principle
%of safe storage [5].
%
%Use formal definition (involving specifying a domain) from Wolf's survey.



%\paragraph{From Wolf Survey and Lecture note.} In the second model, introduced by Cleve and Buhrman [22], Alice and Bob share an unlimited number of EPR-pairs at the start of the protocol, but now they communicate via a classical channel:
%the channel has to be in a classical state throughout the protocol. We only count the communication,
%not the number of EPR-pairs used.  Protocols of this kind can simulate protocols of the ?rst kind
%with only a factor 2 overhead:  using teleportation, the parties can send each other a qubit using
%an EPR-pair and two classical bits of communication. Hence the qubit-protocols that we describe
%below also immediately yield protocols that work with entanglement and a classical channel. Note
%that an EPR-pair can simulate a public coin toss: if Alice and Bob each measure their half of the
%pair of qubits, they get the same random bit.
%
%The third variant combines the strengths of the other two:  here Alice and Bob start out with
%an unlimited number of EPR-pairs and they are allowed to communicate qubits.  This third kind
%of communication complexity is in fact equivalent to the second, up to a factor of 2, again by
%teleportation.
%
%Note that a shared EPR-pair can simulate a public coin toss: ... (My note: Although there is a shared coin, the difference is still that we are allowing error or not.)




%\paragraph{From Buhrman and Buhrman-Rohrig's surveys.} (Section 4.2) (Classical) Communication Complexity was introduced by Yao and Abelson [Abe80, Yao79] ... a three party communication complexity where the three parties share an entangled state, like an EPR-pair but then for three parties.
%
%Kremer [Kre95] and Yao show that the discrepancy bound also works for the ... $Q_2$. This enable them to show ... IP. Ambainis et. al. [ASTS+98] extend this ...  make error which is very close to 1/2. ... For the model where both parties share EPR-pairs, Cleve et. al. [CvDNT98] where the first to show a linear lower bound for IP. ... Theorem 5.

%\paragraph{From Chlebus et al. DISC'10} It is known that quantum communication can be simulated by first distributing entangled pairs of qubits and next sending classical bits, for a cost of two bits per qubit; this mechanism is often called teleportation.

%\paragraph{From Gavoille et al.'09} ... physical
%locality ($\phi$- LOCAL ).  While this is strictly weaker than the computational locality of
%the classical LOCAL model, it nevertheless implies that for many distributed combinatorial
%optimization problems, such as Maximal Independent Set, the best currently known lower
%time bounds cannot be broken by applying quantum processing, in any conceivable way.

%The  quantum  variant  of CONGEST ,  widely studied  in  physics,  is  known  as  the LOCC model. ... [NC00, HHH96] ... starting state entangled among all the processors ... however, communication between processors is still restricted to the exchange of classical information, only.
%
%One especially interesting result is that the leader election problem can be solved in distributed systems with quantum links, but no pre-entanglement [TKM05, KMT08].  Some authors have also claimed that problems related to leader election [PSK03, DP06] and distributed consensus [DP06, Hel08] can be solved in distributed systems aided by quantum pre-entanglement. This paper constitutes an attempt to provide a consistent framework for the aforementioned
%discussions on distributed computing in a quantum setting. ...

%...  a probabilistic framework for proving lower
%bounds on the distributed time complexity of computational problems in any quantum (or other
%unconventional) models based on LOCAL . ...

%... We explain why some of the statements from [PSK03, DP06, Hel08] should be approached with caution ..

%... simply introducing a quantum computer as a module in each processor does not affect the power of the model, since in LOCAL the processors as such are already assumed to have unbounded capabilities of local computation....

%... whenever a problem is solved in a model with the + S extension, it may bene?t solely from the modi?cation of the system initialization, and not from the laws of quantum mechanics ...

%...   Given a general initial state of the system, the outcome of such a physical process, as determined by the processors, may display correlations which cannot be described using any classical probabilistic framework.  ... called non-separable, or entangled states.

%Of course,  the definition of the $^+\cal E$ extension  does not require that the starting  state  is entangled;

%$\cal LOCAL ^+ Q ^+ E$ and $\cal LOCAL ^+ E$ are equivalent in terms of computational power (Proposition 4)

%See Figure 1. Can we say the same thing for CONGEST?

%Quantum relaxations of the $\cal LOCAL$ model, whether obtained through application of pre-entanglement, quantum channels, or both, lie in terms of strength in between the $\cal LOCAL$ and $\phi- \cal LOCAL$ model. ... Theorem 5.

%\paragraph{From Razborov} The definition here is quite rigorous (good!).  ... The models with or without prior entanglement differ only in the choice of ... at the beginning of communication. ... The communication protocol is completely determined by unitary operators ...

%\paragraph{From ...-Chung book} An important two qubit state is the Bell state or EPR pair,...is responsible for many surprises in quantum computation ...That is, the measurement outcomes are correlated. ...  the measurement correlations in the Bell state are stronger than could ever exist between classical systems. ...

%(Section 1.3.3) $|+\rangle$ is used for EPR pair.

%No cloning theorem in Section 1.3.5...  This property, that qubits cannot be copied, is known as the no-cloning theorem, and it is one of the chief differences between quantum and classical information.

%Heres how quantum teleportation works. Alice and Bob met long ago but now live far apart. While to gether they generated an EPR pair, each taking one qubit of the EPR pair when they separated.


%Principle of deferred measurement: Measurementscanalwaysbemovedfrom nintermediatestageofaquantumcircuittotheendofthecircuit;ifthe measurementresultsareusedatanystageofthecircuitthentheclassically controlledoperationscanbereplacedbyconditionalquantumoperations.



%\subsubsection{Quantum Distributed Computing.}

%{\bf (From ``Can Quantum Mechanics Help Distributed Computing?'' (SIGACT)) } One of the most mysterious manifestations of quantum information is entanglement, according to which distant parties can share correlations that go beyond what is feasible with classical information alone: quantum correlations!

%A magic square (see Figure 1)  ... there is no strategy that wins this game with probability more than 8/9.  This is the outcome that the pair of physicists would expect.  Instead, they are astounded to see that Alice and Bob always win, no matter how many times they repeat the game!  ...


%In [23],  ... They exhibited a function (more speci?cally, a relation, also called a promise problem) for three players such that in the broadcast model, ... The function they studied is not very interesting by itself but the result is revolutionary: we knew that entanglement cannot replace communication, and what this result shows is that entanglement can be used to reduce communication in a context of communication complexity.


%... Yao is also responsible for pioneering work in the area of quantum communication complexity [53], in which he asked the question: what if the players are allowed to communicate qubits (quantum information)
%instead of classical bits. No answer to this question was initially advanced. In [23], Richard Cleve and Harry Buhrman introduced a variation on the model, for which they showed a separation between the classical and
%quantum models: the players communicate classically but they share entanglement instead of classical ran-
%dom strings. This time, the goal is to compute the function with certainty. They exhibited a function (more
%speci?cally, a relation, also called a promise problem) for three players such that in the broadcast model,
%any protocol that computes the function requires 3 bits of communication.  In contrast, if the players share
%entanglement, it can be computed exactly with only 2 bits of classical communication.  The function they
%studied is not very interesting by itself but the result is revolutionary: we knew that entanglement cannot re-
%place communication, and what this result shows is that entanglement can be used to reduce communication
%in a context of communication complexity.

%{\bf (From Gopal's SIGACT survey)} Quantum mechanics allows leader election to be solved with no communication, provided that certain pre-shared entanglement is already in place.
%
%The phenomenon of entanglement counter-intuitively invalidates the notion of local realism by creating non-local relationships between quantum objects and blurring the physical state until a measurement is done.
%
%
%Quantum entanglement involves the joint state of two or more qubits.   Informally,  we say that when a
%collection of qubits is entangled, they are non-locally correlated in the sense that performing a measurement
%on one of them instantaneously affects the state of the other(s), even when there are arbitrarily large spatial
%separations between individual qubits.

%There are two types of entanglement that we are interested in for the purposes of distributed computing:
%GHZ [16, 8] and W [8]. ...  2-partite GHZ state (also known as a Bell pair or EPR pair) ...
%
%The restriction of only using classical communication while being able to do
%quantum processing locally is known as Local Operations and Classical Communication (LOCC).  ... This is subsequently referred to as pre-shared entanglement.  No a-priori knowledge is assumed. We refer to this model as LOCC-ENTANGLE. ...QCOMM-ANON.
%
%Tani et al. in [31, 30, 32] assume the QCOMM-ANON model. They show that the general anonymous leader election problem has a correct quantum solution that can be achieved with certainty in polynomial time and communication without assuming any prior entanglement.  Eliminating the dubious entanglement assumption that had to be made in Section 5.2 while still circumventing the classical impossibility for anonymous leader election is a very significant result.


%\fi

